RAMP: Recognition parametrisation by Amortised Message Passing

A central aim of unsupervised learning is to uncover latent factors that explain dependencies among observations. Probabilistic models typically achieve this by introducing multiple latent variables linked through a graph of conditional relationships, with distributional parameters and their dependence learnt from data. Learning relies either on distributional choices that allow tractable belief propagation, or on approximations that scale poorly with model size and complexity. We build on the recently developed recognition-parametrised modelling paradigm to propose an alternative approach: RAMP, a method that implicitly defines latent structure by learning a flexible, nonlinear, amortised message-passing framework. We show that RAMP enables efficient likelihood-based recovery of latent-variable distributions within expressive nonlinear models acting on complex high-dimensional data.

==> m.symbols.tex <==
\RequirePackage{ifthen}
\RequirePackage{etextools}
\RequirePackage{environ}

% use | for math mode
%\catcode`\|=3


%% Misc useful symbols

% use textmode for a shorter minus sign
\newcommand{\tminus}{\text{\textendash}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathbb{E}}{=}}
% conditional independence
\newcommand{\cind}{{\bot\negthickspace\negthickspace\bot}} 
\newcommand{\notcind}{{\smash{\kern0.1em\not\kern-.1em}\cind}}

% isolated fractions
%
% \frac (really \over) places baselines of numerator and denominator to accomodate the normal line
% height and depth.  For an isolated fraction this can look wrong.  \ifrac effectively kills any extra
% space -- at the expense of possibly misaligning baselines in adjacent fracs.
\newcommand{\ifrac}[2]{\mathchoice%
  {\frac{\raisebox{-1ex}{$\textstyle #1$}}{\raisebox{1ex}{$\textstyle #2$}}}%
  {\frac{\raisebox{-1ex}{$\scriptstyle #1$}}{\raisebox{1ex}{$\scriptstyle #2$}}}%
  {\frac{\raisebox{-1ex}{$\scriptscriptstyle #1$}}{\raisebox{1ex}{$\scriptscriptstyle #2$}}}%
  {\frac{\raisebox{-1ex}{$\scriptscriptstyle #1$}}{\raisebox{1ex}{$\scriptscriptstyle #2$}}}%
}
\newcommand{\half}{\ensuremath{\ifrac{1}{2}}}
\newcommand{\thalf}{\ensuremath{\tfrac{1}{2}}}
\newcommand{\overN}{\ensuremath{\tfrac{1}{N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}




%% Utilities to define pretty functions
\makeatletter
\let\x@\expandafter

% Dot-based optional arg control -- useful for indices
%
% \DeclareDotOptCommand\command[nmargs]{nopts}.{opt1}{opt2}...{code}
% Optional nmargs is number of manditory args (before the .)
% Number of opts should equal nopts
% \command.123 reads arguments {1}{2}{3}... (note the leading .)
% \command.1.3 uses default for 2 (applies to any arg)
%   spaces are allowed between args (and around leading .)
%   arg can be a group: \command.{one}{2}
%   if arg starts with a command w/o grouping, it is read to manditory ;: \command.\vec x;2 or \command.\vec{x};2 or \command.\vecx;2
%   if arg is followed by sup/subscripts/primes then these are incorporated into arg
% \command;1;2;3; reads arguments {1}{2}{3}... (note the leading ;)  No arg extensions applied.
% \command (no following .) uses defaults for all
%
% E.g. \DeclareDotOptCommand\XS{2}[i][j]{X_{S_{(#1)(#2)}}} gives
% \XS -> X_{S_{(i)(j)}}
% \XS.jk -> X_{S_{(j)(k)}}
% \XS..k -> X_{S_{(i)(k)}}
% \XS.i{{.}} -> X_{S_{(i)(.)}} -- note double {{}}
% \XS{}. -> X_{S_{(i)(j)}}. but \XS . will read args 

% definition:
\def\DeclareDotOptCommand{\newcommanddotopt}
\def\newcommanddotopt#1{\@ifnextchar[{\newcommanddotopt@{#1}}{\newcommanddotopt@{#1}[0]}}
\def\newcommanddotopt@#1[#2]#3.{
  \edef\dotopt@cmd{\x@\@gobble\string#1}
  \edef#1{\noexpand\dotopt@exec{\dotopt@cmd}}%
  \csdef{dotopt@\dotopt@cmd @nummargs}{#2}%
  \csdef{dotopt@\dotopt@cmd @numopts}{#3}%
  \dotopt@getdefaults@next{\dotopt@cmd}{1}{#3}%
}
\def\dotopt@getdefaults@next#1#2#3{\ifnumgreater{#2}{#3}{\dotopt@getcode{#1}{#3}}{\dotopt@getdefaults@read{#1}{#2}{#3}}}
\def\dotopt@getdefaults@read#1#2#3#4{\csgdef{dotopt@#1@default#2}{#4}\dotopt@getdefaults@next{#1}{\the\numexpr #2+1\relax}{#3}}
\def\dotopt@getcode#1#2#3{%
  \x@\newcommand\csname dotopt@#1@code\endcsname[\numexpr #2+\csuse{dotopt@#1@nummargs}\relax]{#3}}

% execution: 
\def\dotopt@exec#1{\dotopt@get@margs@next{#1}{1}{}}
\def\dotopt@get@margs@next#1#2#3{%
  \ifnumless{#2}{\csuse{dotopt@#1@nummargs}+1}%
    {\dotopt@get@margs@read{#1}{#2}{#3}}
    {\@ifnextchar.{\dotopt@get@opts@next@dot{#1}{1}{#3}}
      {\@ifnextchar;{\dotopt@get@opts@next@semi{#1}{1}{#3}}
        {\dotopt@exec@defaults{#1}{1}{#3}}}}
}
\def\dotopt@get@margs@read#1#2#3#4{\dotopt@get@margs@next{#1}{#2+1}{#3{#4}}}

\def\dotopt@get@opts@next@semi#1#2#3;#4#5;{%
  \ifnumless{#2}{\csuse{dotopt@#1@numopts}}
    {\ifstrequal{#4}{.}
      {\dotopt@get@opts@next@semi{#1}{#2+1}{#3{\csuse{dotopt@#1@default\the\numexpr#2\relax}#5}};}
      {\dotopt@get@opts@next@semi{#1}{#2+1}{#3{#4#5}};}}
    {\ifstrequal{#4}{.}
      {\dotopt@exec@{#1}{#3{\csuse{dotopt@#1@default\the\numexpr#2\relax}#5}}}%
      {\dotopt@exec@{#1}{#3{#4#5}}}}%
}

\def\dotopt@get@opts@next@dot#1#2#3.{%
  \ifnumless{#2}{\csuse{dotopt@#1@numopts}+1}{\dotopt@get@opts@read{#1}{#2}{#3}}{\dotopt@exec@{#1}{#3}}%
}
\def\dotopt@get@opts@read#1#2#3#4{%
  % is arg a macro? see https://tex.stackexchange.com/a/21887
  \if\noexpand#4\relax\x@\@firstoftwo\else\x@\@secondoftwo\fi{
    \dotopt@get@opts@command{#1}{#2}{#3}#4%
  }{%
    \ifstrequal{#4}{(}{\dotopt@get@opts@paren{#1}{#2}{#3}#4}{%
      \ifstrequal{#4}{[}{\dotopt@get@opts@brack{#1}{#2}{#3}#4}{%
        \dotopt@get@opts@chkss{#1}{#2}{#3}{#4}{}%
  }}}%
}
\def\dotopt@get@opts@command#1#2#3#4;{\dotopt@get@opts@next@dot{#1}{#2+1}{#3{#4}}.}
\def\dotopt@get@opts@chkss#1#2#3#4#5{%
  \@ifnextchar'{\dotopt@get@opts@prime{#1}{#2}{#3}{#4}{#5}}{%
    \@ifnextchar_{\dotopt@get@opts@sub{#1}{#2}{#3}{#4}{#5}}{%
      \@ifnextchar^{\dotopt@get@opts@sup{#1}{#2}{#3}{#4}{#5}}{%
        \ifstrequal{#4}{.}
          {\dotopt@get@opts@next@dot{#1}{#2+1}{#3{\csuse{dotopt@#1@default\the\numexpr#2\relax}#5}}.}%
          {\dotopt@get@opts@next@dot{#1}{#2+1}{#3{#4#5}}.}%
  }}}
}
\def\dotopt@get@opts@paren#1#2#3(#4){\dotopt@get@opts@chkss{#1}{#2}{#3}{(#4)}{}}
\def\dotopt@get@opts@brack#1#2#3[#4]{\dotopt@get@opts@chkss{#1}{#2}{#3}{[#4]}{}}
\def\dotopt@get@opts@prime#1#2#3#4#5'{\dotopt@get@opts@chkss{#1}{#2}{#3}{#4}{#5'}}
\def\dotopt@get@opts@sub#1#2#3#4#5_#6{\dotopt@get@opts@chkss{#1}{#2}{#3}{#4}{#5_{#6}}}
\def\dotopt@get@opts@sup#1#2#3#4#5^#6{\dotopt@get@opts@chkss{#1}{#2}{#3}{#4}{#5^{#6}}}

\def\dotopt@exec@defaults#1#2#3{%
  \ifnumgreater{#2}{\csuse{dotopt@#1@numopts}}
    {\dotopt@exec@{#1}{#3}}
    {\dotopt@exec@defaults{#1}{#2+1}{#3{\csuse{dotopt@#1@default\the\numexpr#2\relax}}}}
}
\def\dotopt@exec@#1#2{\csuse{dotopt@#1@code}#2}


%\newcommand\optly[3]{\ExpandNext\@ifempty{#1}{#3}{#2}}
\newcommanddotopt\optly[1]{2}.{}{}{\expandselect{\@ifempty`##{#1}`}{#3}{#2}}

% Functions with resizeable delimiters
%
% \DeclareResizableDelimFunction{macroname}{symbol}{left delim}{right delim}
%
% E.g. \DeclareResizableDelimFunction{foo}{\text{foo}}[]
% defines:
% \foo{x} -> \text{foo} \left[ x \right]
% \foo[\big]{x} -> \text{foo} \big[ x \big]
\def\DeclareResizableDelimFunction#1#2#3#4{
  \x@\newcommand\csname#1\endcsname[2][*]{%
    #2\lr[##1]#3#4{##2}}}

% \DeclareResizableDelimFunction{macroname}{symbol}{left delim}{right delim}{separator}
%
% E.g. \DeclareResizableDelimFunction{foo}{\text{foo}}[]{,}
% defines:
% \foo{x}{y} -> \text{foo} \left[ x , y\right]
% \foo[\big]{x}{y} -> \text{foo} \big[ x , y \big]
%
% \DeclareResizableDelimFunction{foo}{\text{foo}}[]{\lrmid \|}
% defines:
% \foo{x}{y} -> \text{foo} \left[ x \middle \|  y\right]
% \foo[\big]{x}{y} -> \text{foo} \big[ x \big \|  y \big]
\def\DeclareResizableDelimFunctionOnTwoArgs#1#2#3#4#5{
  \x@\newcommand\csname#1\endcsname[3][*]{%
    #2\lr[##1]#3#4{##2 #5 ##3}}}

% Optional subscripted functions with resizeable delimiters
%
% \DeclareOptSubscriptedFunction{macroname}{symbol}[default subscr]{left delim}{right delim}
%
% E.g. \DeclareOptSubscriptedFunction{foosq}{\text{foo}^2}[][]
% defines:
% \foosq{x} -> \text{foo}^2 \left[ x \right]
% \foosq[a]{x} -> \text{foo}^2_a \left[ x \right]
% \foosq[a][\big]{x} -> \text{foo}^2_a \big[ x \big]
% \foosq[][\big]{x} -> \text{foo}^2 \big[ x \big]
% \foosq[][][()]{x} -> \text{foo}^2 \left ( x \right )
% Note that _{} would normally add undesirable space that this definition avoids
\def\OptSubscript#1{\ifthenelse{\equal{#1}{}}{}{_{#1}}}
\def\DeclareOptSubscriptFunction#1#2[#3]#4#5{
  \x@\def\csname#1\endcsname{%
    \@ifnextchar[{\csname#1@\endcsname}{\csname#1@@@\endcsname[#3][*][{#4}{#5}]}}
  %
  \x@\def\csname#1@\endcsname[##1]{%
    \@ifnextchar[{\csname#1@@\endcsname[##1]}{\csname#1@@@\endcsname[##1][*][{#4}{#5}]}}
  %
  \x@\def\csname#1@@\endcsname[##1][##2]{%
    \@ifnextchar[{\csname#1@@@\endcsname[##1][##2]}{\csname#1@@@\endcsname[##1][##2][{#4}{#5}]}}
  %
   \x@\def\csname#1@@@\endcsname[##1][##2][##3##4]##5{%
%               {\ensuremath{#2\OptSubscript{##1}|##2|##3|##4|##5|}}}
               {\ensuremath{#2\OptSubscript{##1}\lr[##2]{##3}{##4}{##5}}}}
}
\def\DeclareOptSubscriptOptArgFunction#1#2[#3]#4#5{
  \x@\def\csname#1\endcsname{%
    \@ifnextchar[{\csname#1@\endcsname}{\csname#1@@@\endcsname[#3][*][{#4}{#5}]}}
  %
  \x@\def\csname#1@\endcsname[##1]{%
    \@ifnextchar[{\csname#1@@\endcsname[##1]}{\csname#1@@@\endcsname[##1][*][{#4}{#5}]}}
  %
  \x@\def\csname#1@@\endcsname[##1][##2]{%
    \@ifnextchar[{\csname#1@@@\endcsname[##1][##2]}{\csname#1@@@\endcsname[##1][##2][{#4}{#5}]}}
  %
   \x@\def\csname#1@@@\endcsname[##1][##2][##3##4]##5{%
     \ifthenelse{\equal{##5{}}{{}}}% if arg is empty omit delimeters
                {\ensuremath{#2\OptSubscript{##1}}}%
                {\ensuremath{#2\OptSubscript{##1}\lr[##2]{##3}{##4}{##5}}}}
}

\makeatother


% probability distributions
%\DeclareOptSubscriptOptArgFunction{pr}{{\bf\sf{P}}}[]()
% \DeclareOptSubscriptFunction{prf}{\bf\sf{P}}[]{}{}

% \newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
% \newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
% \newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}

% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\size]{x} -> \mathbb{E}_a \size[ x \size]
% \DeclareOptSubscriptFunction{expect}{\mathbb{E}}[][]
\DeclareOptSubscriptFunction{var}{\mathbb{V}}[][]
% \DeclareResizableDelimFunction{angles}{}\langle\rangle

% likelihoods
\DeclareOptSubscriptFunction{like}{\mathcal{L}}[]()
\DeclareOptSubscriptFunction{loglike}{\ell}[]()

% info theoretic
\DeclareResizableDelimFunction{entropy}{\textbf{\textsf{H}}}[]
\DeclareResizableDelimFunctionOnTwoArgs{info}{\textbf{\textsf{I}}}[]{\mathbin{;}}
\def\mutualinfo[#1;#2]{\info{#1}{#2}} % older form
% \DeclareResizableDelimFunctionOnTwoArgs{KL}{\textbf{\textsf{KL}}}[]{\lrmid\|}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
% \DeclareResizableDelimFunctionOnTwoArgs{normal}{\mathcal{N}}(){,}

% whitened quantities
% \newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}
% explicitly defined in some old versions
% \newcommand{\setV}{\ensuremath{{\cal V}}}
% \newcommand{\setX}{\ensuremath{{\cal X}}}
% \newcommand{\setY}{\ensuremath{{\cal Y}}}
% \newcommand{\setZ}{\ensuremath{{\cal Z}}}
\DeclareResizableDelimFunction{size}{}\vert\vert

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
% bm seems to do what we need without overt mode switches
\usepackage{bm}
\renewcommand{\vec}[1]{\bm{\mathsf{#1}}}
% \renewcommand{\vec}[1]{\ensuremath{\mathchoice%
% {\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
% {\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
% {\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
% {\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
%\DeclareResizableDelimFunction{norm}{}\|\|
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\let\det\undefined % lose std definition
\DeclareResizableDelimFunction{det}{}\vert\vert
\DeclareResizableDelimFunction{trace}{\mathsf{Tr}}[]
\DeclareResizableDelimFunction{diag}{\mathbox{\textsf{diag}}}[]

% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\MDeriv}[3][]{\frac{d^{#1}{#2}}{{d#3}^{#1}}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\makeatletter
\newcommand{\@dx}[1][dx]{%
  \mathchoice{\mkern-3mu}{}{}{}% extra backkern in display
  \mkern-3mu#1\,% 
}
\newcommand{\intdx}[1][dx]{\int\@dx[#1]}
\newcommand{\intinf}{\int_{-\infty}^{+\infty}}
\newcommand{\intinfdx}[1][dx]{\int_{-\infty}^{+\infty}\@dx[#1]}



% \mltint -> \int\dots\int with better spacing
% \mltint[3] -> \int\int\int with better spacing
% more compact than amsmath \iint \iiint \idotsint 
\newcounter{multintctr}
\newcommand{\mltint}[1][]{%
  \ifthenelse{\equal{#1{}}{{}}}
    {\int\mkern-6mu{\cdot} %{} kills default space around \cdot
      \mathchoice%
        {\mkern1mu{\cdot}\mkern1mu}% display
        {{\cdot}}% inline
        {{\cdot}}% script
        {{\cdot}}% sscript
      {\cdot}\mkern-6mu}
    {\setcounter{multintctr}{1}%
      \whiledo{\value{multintctr}<#1}{%
        \int\mkern-12mu%
        \stepcounter{multintctr}%
      }}%
    \int}

\def\mltintdx{%
  \@ifnextchar[{\@mltintdx}{\@mltintdx[]}%
}
\def\@mltintdx[#1]{\mltint[#1]\@dx}

\makeatother

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
%\newcommand{\complexes}{\mathbb{C}}
%\newcommand{\reals}{\mathbb{R}}
%\newcommand{\integers}{\mathbb{Z}}
%\newcommand{\naturalss}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}




% accents

% from symbols-a4.pdf; optional arg permits shortening to prevent
% adjacent bars running together
\newcommand{\widebar}[2][3]{{}\mkern#1mu\overline{\mkern-#1mu#2}}

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}

\makeatletter

%% 
%% expandselect
%%

% \expandselect{input} processes <input>, expanding material between ``s as follows:
% `<text>` - expand first token in <text> (may read following arguments from <text>)
% `!<text>` - expand all expandable tokens in <text> fully using \edef
% `#<mtext>` - expand <mtext> (respecting additional modifiers), group result in {}s
% `&<mtext>` - expand <mtext> (respecting additional modifiers), then expand first token of result
% `>{<etext>}` - effectively \expandselect{<etext>} (grouping is removed unless preceded by #)
%
% <mtext> may start with modifiers:
% `#!<text>` - expand fully and group
% `#>{foo `\bar`}` -> {foo <bar expanded>}
% `##&&\bar` - expand bar three times and group twice
%
% Both [&#]{<mtext>} effectively run \expandselect{`<mtext>`}.  So behaviour is modified by any
%   (explicit) ` characters in <mtext>
% `&{`\foo`\bar}` -> ``\foo`\bar`, expanding \bar (and then \foo).
% `&>{`\foo`\bar}` expands \foo twice (as does `&\foo\bar`)
%
% \expandafter, \noexpand, \unexpanded can be used within <text>
% `&\expandafter\foo\bar` -> <foo expanded second><bar expanded first> (so \foo can process tokens in \bar replacement text)
% Here `&>{\foo`\bar`}` has the same effect, but consider:
% `&&>{\expandafter`\foobar`}` where \foobar->\foo\bar
%
% Expansion chars (`) must appear explicitly in <input>.  Chars generated from expansions are not processed.
%
% Expansion char may be changed with option: \expandselect[|]{text|expand|}, but cannot (sensibly) be #,!,&, or >.
%
% \expandselect is not expandable, so cannot be nested
%
% BUG?: \expandselect{`\foo{bar}`} drops the grouping of {bar}.  Workaround: \expandselect{`{}\foo{bar}`}
% FIXED?: needs more testing


\newtoks\mmt@xpsel@toks         %collect (expanded) tokens
\newtoks\toks@@                 %tmp register
\def\appendtoks#1#2{#1=\x@{\the#1#2}}

\newcommand\expandselect[2][`]{%
  \mmt@xpsel@defparser{#1}\mmt@xpsel{#2}%
}
\def\mmt@xpsel@defparser#1{%
  \def\mmt@xpsel##1{%
    \mmt@xpsel@toks={}\mmt@xpsel@parse\mmt@xpsel@toks @##1#1@#1@@% @##1 avoids losing {} around ##1
%    \showthe\mmt@xpsel@toks% for debugging
    \the\mmt@xpsel@toks}%
  % \def\mmt@xpsel@parse##1##2#1##3##4#1##5@@{% toks;unexpanded;modifier?;expand text;remain
  %   \x@\appendtoks\x@##1\x@{\@gobble##2}% discard {}-preserving @
  %   \ifx @##3\relax\x@\@firstoftwo\else\x@\@secondoftwo\fi{%
  %     % done parsing
  %   }{\ifstrequal{##3}{#1}{% #1#1 in input - expand to nothing and continue
  %       \mmt@xpsel@parse##1@##4#1##5@@% ##4#1 was taken from remaining text
  %     }{%
  %       \ifstrequal{##3}{####}{%
  %         \begingroup%
  %         \toks@@={}\ifblank{##4}{}{\mmt@xpsel@parse{\toks@@}@#1##4#1#1@#1@@}%
  %         \xdef\mmt@xpsel@tmp{\the\toks@@}% xdef will only expand token register once
  %         \endgroup%
  %         \x@\appendtoks\x@##1\x@{\x@{\mmt@xpsel@tmp}}}{%
  %       \ifstrequal{##3}{!}{%
  %         \edef\mmt@xpsel@tmp{##4}%
  %         \x@\appendtoks\x@##1\x@{\mmt@xpsel@tmp}}{%
  %       \ifstrequal{##3}{>}{%
  %         \begingroup%
  %         \toks@@={}\mmt@xpsel@parse{\toks@@}@##4#1@#1@@%
  %         \xdef\mmt@xpsel@tmp{\the\toks@@}% xdef will only expand token register once
  %         \endgroup%
  %         \x@\appendtoks\x@##1\x@{\mmt@xpsel@tmp}}{%
  %       \ifstrequal{##3}{&}{%
  %         \begingroup%
  %         \toks@@={}\mmt@xpsel@parse{\toks@@}@#1##4#1#1@#1@@%
  %         \xdef\mmt@xpsel@tmp{\the\toks@@}% xdef will only expand token register once
  %         \endgroup%
  %         \x@\x@\x@\appendtoks\x@\x@\x@##1\x@\x@\x@{\mmt@xpsel@tmp}%
  %       }{% no modifier, ##3 is part of expansion text
  %         \x@\appendtoks\x@##1\x@{##3##4}%
  %       }}}}%
  %       \mmt@xpsel@parse##1@##5@@% parse the remaining text
  %     }%
  %   }%
  % }%
  \def\mmt@xpsel@parse##1##2#1##3#1##4@@{% toks;unexpanded;modifier?-expand text;remain
    \x@\appendtoks\x@##1\x@{\@gobble##2}% discard {}-preserving @
    \ifx @##3\relax\x@\@firstoftwo\else\x@\@secondoftwo\fi{%
      % done parsing
    }{\ifblank{##3}{}{% #1#1 in input - expand to nothing and continue
        \if@mmt@xpsel@mod##3@{%
          \mmt@xpsel@xpnd@mod##1##3@% expand modifier
        }{%
          \x@\appendtoks\x@##1\x@{##3}% no modifier, just expand
        }%
      }%
      \mmt@xpsel@parse##1@##4@@% parse the remaining text
    }%
  }%
  \def\mmt@xpsel@xpnd@mod##1##2##3@{%
    \ifstrequal{##2}{####}{%
      \begingroup%
      \toks@@={}\ifblank{##3}{}{\mmt@xpsel@parse{\toks@@}@#1##3#1#1@#1@@}%
      \xdef\mmt@xpsel@tmp{\the\toks@@}% xdef will only expand token register once
      \endgroup%
      \x@\appendtoks\x@##1\x@{\x@{\mmt@xpsel@tmp}}}{%
    \ifstrequal{##2}{!}{%
      \edef\mmt@xpsel@tmp{##3}%
      \x@\appendtoks\x@##1\x@{\mmt@xpsel@tmp}}{%
    \ifstrequal{##2}{>}{%
      \begingroup%
      \toks@@={}\mmt@xpsel@parse{\toks@@}@##3#1@#1@@%
      \xdef\mmt@xpsel@tmp{\the\toks@@}% xdef will only expand token register once
      \endgroup%
      \x@\appendtoks\x@##1\x@{\mmt@xpsel@tmp}}{%
    \ifstrequal{##2}{&}{%
      \begingroup%
      \toks@@={}\mmt@xpsel@parse{\toks@@}@#1##3#1#1@#1@@%
      \xdef\mmt@xpsel@tmp{\the\toks@@}% xdef will only expand token register once
      \endgroup%
      \x@\x@\x@\appendtoks\x@\x@\x@##1\x@\x@\x@{\mmt@xpsel@tmp}%
    }{\x@\appendtoks\x@##1\x@{##2##3}}% unrecognised modifier, just expand
    }}}%
  }%
}%

\def\if@mmt@xpsel@mod#1#2@{\begingroup
  \edef\x{\endgroup\noexpand\in@{\detokenize{#1}}{\detokenize{##!>&}}}%
  \x\ifin@\x@\@firstoftwo\else\x@\@secondoftwo\fi%
}

        

%% 
%% moving subscripts
%%

\def\withscripts#1{\mmt@withscripts{#1}{}}
% \def\mmt@withscripts#1#2{%
%   \@ifchar{_}{\mmt@withscripts@two{#1}{#2}_}{%
%     \@ifchar{^}{\mmt@withscripts@two{#1}{#2}^}{%
%       \@ifchar'{\mmt@withscripts@one{#1}{#2}'}{%
%         \@ifchar{\limits}{\mmt@withscripts@one{#1}{#2}\limits}{%
%           \@ifchar{\nolimits}{\mmt@withscripts@one{#1}{#2}\nolimits}{%
%             #1{#2}%
%   }}}}}%
% }
\def\mmt@withscripts#1#2{%
  \@ifnextchar_{\mmt@withscripts@two{#1}{#2}}{%
    \@ifnextchar^{\mmt@withscripts@two{#1}{#2}}{%
      \@ifnextchar'{\mmt@withscripts@one{#1}{#2}}{%
        \@ifnextchar\limits{\mmt@withscripts@one{#1}{#2}}{%
          \@ifnextchar\nolimits{\mmt@withscripts@one{#1}{#2}}{%
            #1{#2}%
  }}}}}%
}
\def\mmt@withscripts@one#1#2#3{\mmt@withscripts{#1}{#2#3}}
\def\mmt@withscripts@two#1#2#3#4{\mmt@withscripts{#1}{#2#3{#4}}}

\def\afterscripts#1{\withscripts{\@swap{#1}}}

%% overrideable left-right delimeters


% compare #1 to first token of #2, if equal -> #3 else ->#4
\long\def\iffirstx#1#2#3#4{\@ifempty{#2}{#4}{\x@\@iffirstx\x@#1#2@{#3}{#4}}}
\long\def\@iffirstx#1#2#3@#4#5{\ifx#1#2\x@\@firstoftwo\else\x@\@secondoftwo\fi{#4}{#5}}
\long\def\iffirst#1#2#3#4{\@ifempty{#2}{#4}{\x@\@iffirst\x@#1\detokenize{#2}@{#3}{#4}}}
\long\def\@iffirst#1#2#3@#4#5{\if#1#2\x@\@firstoftwo\else\x@\@secondoftwo\fi{#4}{#5}}
\long\def\ifsecond#1#2#3#4{\@ifempty{#2}{#4}{\x@\@ifsecond\x@#1\detokenize{#2}@{#3}{#4}}}
\long\def\@ifsecond#1#2#3#4@#5#6{\@ifempty{#3}{#6}{\if#1#3\x@\@firstoftwo\else\x@\@secondoftwo\fi{#5}{#6}}}


%% 
%% lr:
%% 
% \lr(){foo} -> \left(foo\right)
% \lr[\big](){foo} -> \big({foo}\big)
% \lr[=3ex](){foo} -> explicit size
% \lr[=2ex:1ex](){foo} -> explicit size (above:below) math axis
% \lr[~\sum](){foo} -> size delimiters as though (only) argument was \sum
% \lr[][]{foo} -> \left[{foo}\right]  -- double [] to avoid delims begin processed as (empty) opt
% \lr\{\}{a \lrmid | b } will re-scale the `|' appropriately
% \lr..{foo} -> \left. foo \right. -- no delims but \lrmid will still work
% \lr{}{}{foo} -> foo -- no delims (and lrmid won't work), useful when lr is called from other macros
% this version should nest correctly.  

\usepackage{mleftright}
\mleftright

\newcommand\lrdefault[1][*]{\def\lr@default{#1}}
\lrdefault

\newcommand\lr[4][-]{%
  \ifblank{#2#3}{#4}{%
    \begingroup% limit scope of \defs
    \ifblank {#1}{% 
      \lr@lr{}[]{#2}\AfterGroup{#3#4}}{%
    \ifstrequal -{#1}{%
      \x@\lr\x@[\lr@default]{#2}{#3}{#4}}{%
    \ifstrequal *{#1}{%
      \lr@lr{#1}{#2}{#3}{#4}}{%
    \iffirst ={#1}{%
      \lr@setbox\lr@box#1::@%
      \lr@set{\copy\lr@box}{#2}{#3}{#4}}{%
    \iffirst :{#1}{%
      \ifstrequal{:}{#1}{% just : => natural size
        \lr@max@palette<:50ex@{#2}{#3}{#4}% => <: a large size
      }{%
        \lr@setbox\lr@box#1::@%
        \lr@set@adj{#1}{\vcenter{\copy\lr@box}}{#2}{#3}{#4}}%
    }{%
    \x@\iffirst\string~{#1}{%
      \lr@set{\lr@vphantom#1@}{#2}{#3}{#4}}{%
    \iffirst >{#1}{%
      \ifsecond ={#1}{%
        \expandselect{\lr@setbox\lr@box`\@gobble#1`::@}%
        \lr@min{\copy\lr@box}{#2}{#3}{#4}}{%
      \x@\ifsecond \string~{#1}{%
        \lr@min{\x@\lr@vphantom\@gobble#1@}{#2}{#3}{#4}%
      }{% otherwise
        \lr@min{\lr@vphantom#1.@}{#2}{#3}{#4}%
      }}}{%
    \iffirst <{#1}{%
      \lr@max@palette#1@{#2}{#3}{#4}%
    }{% otherwise
      \lr@cmd{#1}{#2}{#3}{#4}%
    }}}}}}}}%
    \endgroup%
  }%
}

%% HACK: 12/6/25 -- texlive version 2023.20240207
%% we need to test for \big etc by expanding to check if they start with the ams command \bBigg@.
%% At some point amsmath redefined the sizing macros with \DeclareRobustCommand which prevents
%% expansion.  This goes back to the earlier definition -- has risk of side effects.
\renewcommand{\big}{\bBigg@\@ne}
\renewcommand{\Big}{\bBigg@{1.5}}
\renewcommand{\bigg}{\bBigg@\tw@}
\renewcommand{\Bigg}{\bBigg@{2.5}}

\newif\if@lropt
\def\@iflropt#1{%
  \@lroptfalse%
  \ifblank{#1}{}{%
  \ifstrequal -{#1}{\@lropttrue}{%
  \ifstrequal *{#1}{\@lropttrue}{%
  \iffirst ={#1}{\@lropttrue}{%
  \iffirst :{#1}{\@lropttrue}{%
  \x@\iffirst\string~{#1}{\@lropttrue}{%
  \iffirst >{#1}{\@lropttrue}{%
  \iffirst <{#1}{\@lropttrue}{%
  \iffirstx\bBigg@{#1}{\@lropttrue}{%
  }}}}}}}}}%
  \if@lropt\x@\@firstoftwo\else\x@\@secondoftwo\fi%
}

\def\@fixdotsp{\kern-\nulldelimiterspace}
\def\lr@cmd#1#2#3#4{\def\lrmid{#1} \mathopen#1#2#4\mathclose#1#3}
\def\lr@lr#1#2#3#4{\let\lrmid\middle\left#2#4\right#3}
\def\lr@set#1#2#3#4{\def\lrmid##1{\left.\@fixdotsp#1\middle##1\right.\@fixdotsp}%
  \left#2#1\right.\@fixdotsp#4\left.\@fixdotsp#1\right#3}
\def\lr@set@adj#1#2#3#4#5{\def\lrmid##1{\lr@vadj#1::@{\left.\@fixdotsp#2\middle##1\right.\@fixdotsp}}%
  \lr@vadj#1::@{\left#3#2\right.\@fixdotsp}#5\lr@vadj#1::@{\left.\@fixdotsp#2\right#4}}
\def\lr@min#1#2#3#4{\let\lrmid\middle\left#2#1#4\right#3}


\def\lr@max@palette<#1@#2#3#4{\mathpalette\lr@max@palette@{#1@{#2}{#3}{#4}}}
\def\lr@max@palette@#1#2{\lr@max@parse#1#2}
\def\lr@max@parse#1#2#3@#4#5#6{%
  \setbox\z@\hbox{$\m@th#1{\def\lrmid{}#6}$}%
  \ifstrequal{=}{#2}{\lr@setbox\tw@=#3::@}{%
    \ifstrequal{:}{#2}{\lr@setbox\tw@:#3::@}{%
      \ifstrequal{~}{#2}{\setbox\tw@\hbox{$\m@th#1 #3$}}{%
        \setbox\tw@\hbox{$\m@th#1 #2.$}}}}%
  \setbox\lr@box\null%
  \ifdimless{\ht\z@}{\ht\tw@}{\ht\lr@box\ht\z@}{\ht\lr@box\ht\tw@}%
  \ifdimless{\dp\z@}{\dp\tw@}{\dp\lr@box\dp\z@}{\dp\lr@box\dp\tw@}%
  \ifstrequal{:}{#2}%
    {\lr@set@adj{:\ht\lr@box-\m@axis:\dp\lr@box+\m@axis}{\vcenter{\copy\lr@box}}{#4}{#5}{#6}}%
    {\lr@set{\copy\lr@box}{#4}{#5}{#6}}%
}

% a box for lr control
\newbox\lr@box
% math axis height: https://tex.stackexchange.com/a/618057
\def\m@axis{\fontdimen22\textfont2}

\def\lr@setbox#1#2#3:#4:#5@{% box=ht:dp::@ OR box=ht::@
  \setbox#1\null%
  \ifblank{#4}%
    {\ht#1\dimexpr#3/2+\m@axis \dp#1\dimexpr#3/2-\m@axis\relax}%
    {\ht#1\dimexpr#3+\m@axis \dp#1\dimexpr#4-\m@axis\relax}%
}
\def\lr@vadj:#1:#2:#3@#4{% =ht:dp:0pt:\end /=ht:0pt:\end
  \def\@vadj##1##2{\raisebox{\dimexpr((#1)-(#2))/2}{$\m@th##1 ##2$}}% \m@th->\mathsurround0pt
  \ifblank{#2}{#4}{{\mathpalette\@vadj{#4}\vrule width0pt}}% vrule puts su*scripts in correct places
}
\def\lr@vphantom#1#2@{\vphantom{#2}}


\def\lr@rule#1#2:#3:#4@#5{% =ht:dp::@ /=ht::@
  \ifblank{#3}
    {\vcenter{\hrule height\dimexpr#2 depth0pt width\dimexpr#5\relax}}
    {\vrule height\dimexpr#2+\m@axis depth\dimexpr#3-\m@axis width\dimexpr#5\relax}%
}
\newcommand\lrvrule[2][0.4pt]{\lr@rule=#2::@{#1}}


%%
%% \DeclareLRCommand\name\ldelim\rdelim
%% \DeclareLRCommand\name[nargs][opt]\ldelim\rdelim{code}
%% \DeclareLRCommand\name[nargs][opt]\ldelim\rdelim[prefix]{code}[suffix]
%% \DeclareLRCommand\name[nargs][opt]\ldelim\rdelim*{\LR code}
%%

\def\DeclareLRCommand#1{%
  \def#1{\@ifnextchar[{\lr@call@opt#1}{\lr@call@noopt#1}}% the eventual invocation 
  \@ifnextchar[{\@lr@command@arg{#1}}{\@lr@command@noarg{#1}}}% look for arg definition
%% definition has no arguments
\def\@lr@command@noarg#1#2#3{%
  \@lr@command@args#1{[1]}#2#3{##1}}
%% definition has arguments
\def\@lr@command@arg#1[#2]{%
  \@ifempty{#2}{\@lr@command@noarg{#1}[]}{% ifempty then [] are delimiters, not arg defn
    \@ifnextchar[{\@lr@command@arg@opt{#1}[#2]}{\@lr@command@args{#1}{[#2]}}}}%
\def\@lr@command@arg@opt#1[#2][#3]{\@lr@command@args{#1}{[#2][#3]}}%
\def\@lr@command@args#1#2#3#4{\@ifstar{\@lr@command@args@star{#1}{#2}{#3}{#4}}{\@lr@command@args@nostar{#1}{#2}{#3}{#4}}}
\def\@lr@command@args@star#1#2#3#4#5{%
  \x@\newcommand\csname lrcmd@\string#1\endcsname#2{{\def\LR{\x@\lr\x@[\lr@default@this]{#3}{#4}}#5}}}
\def\@lr@command@args@nostar#1#2#3#4{%
  \@ifnextchar[{\@lr@command@args@prefix{#1}{#2}{#3}{#4}}{\@lr@command@args@prefix{#1}{#2}{#3}{#4}[]}}
\long\def\@lr@command@args@prefix#1#2#3#4[#5]#6#7{% long because #7 might be \par
  \if[#7\x@\@firstoftwo\else\x@\@secondoftwo\fi%
    {\@lr@command@args@suffix{#1}{#2}{#3}{#4}[#5]{#6}[}%
    {\x@\newcommand\csname lrcmd@\string#1\endcsname#2{#5\x@\lr\x@[\lr@default@this]{#3}{#4}{#6}}#7}}
\def\@lr@command@args@suffix#1#2#3#4[#5]#6[#7]{%
  \x@\newcommand\csname lrcmd@\string#1\endcsname#2{#5\x@\lr\x@[\lr@default@this]{#3}{#4}{#6}#7}}
%% invoke the defined function
\def\lr@call@noopt#1{\def\lr@default@this{-}\csuse{lrcmd@\string#1}}
\def\lr@call@opt#1[#2]{%
  \@iflropt{#2}%
    {\def\lr@default@this{#2}\csuse{lrcmd@\string#1}}%
    {\@ifnextchar[{\lr@call@twoopt#1[#2]}{\def\lr@default@this{-}\csuse{lrcmd@\string#1}[#2]}}%
}
\def\lr@call@twoopt#1[#2][#3]{\def\lr@default@this{#3}\csuse{lrcmd@\string#1}[#2]}


\def\optsub#1{\@ifempty{#1}{}{_{#1}}}
\def\optsup#1{\@ifempty{#1}{}{^{#1}}}

\DeclareLRCommand\angles\langle\rangle
\DeclareLRCommand\abs||
\DeclareLRCommand\bra\langle|
\DeclareLRCommand\ket|\rangle
\DeclareLRCommand\braket[2]\langle\rangle{#1\lrmid|#2}
\DeclareLRCommand\brack[]
\DeclareLRCommand\commutator[2]\lbrack\rbrack{#1,#2}
\DeclareLRCommand\norm[2][]\|\| {#2}[\optsub{#1}]
\DeclareLRCommand\pr[2][]()*{\mathsf{P}\optsub{#1}\LR{#2}}
% \DeclareLRCommand\expect[2][]\lbrack\rbrack[\mathbb{E}\optsub{#1}]{#2}
\DeclareLRCommand\KL[2]\lbrack\rbrack[\textbf{\textsf{KL}}]{#1\lrmid\|#2}
%\DeclareLRCommand\normal[3]()[\mathcal{N}]{#1,#2}


%% 
%% \lrify
%%

% if macro, replace leading char with '@'
\def\delim@name#1{\if\noexpand#1\relax\x@\@firstoftwo\else\x@\@secondoftwo\fi{@\x@\@gobble\string#1}{#1}}

\newcommand\DeclareLRDelimPair[2]{%
  \def\d@l{\delim@name}% just for compactness
  \csdef{delim@close@\d@l#1}{#2}%
  \csdef{lr@close@\d@l#1}{%
    \global\delimited@toks=\x@{\the\delimited@toks#2}%
    \csuse{delim@scantoclose@\d@l#1}}%
  \csdef{delim@scantoclose@\d@l#1}##1#2{\csuse{delim@scanforopen@\d@l#1}##1#1@\@end}%
  \csdef{delim@scanforopen@\d@l#1}##1#1##2##3\@end{%
    \if @##2\x@\@firstoftwo\else\x@\@secondoftwo\fi%
      {\global\delimited@toks=\x@{\the\delimited@toks##1}\endgroup}
      {\global\delimited@toks=\x@{\the\delimited@toks##1#1}%
        \begingroup\x@\aftergroup\csname lr@close@\d@l#1\endcsname\csuse{delim@scanforopen@\d@l#1}##2##3\@end}}%
}

\def\ifpaireddelim#1{\ifcsdef{delim@close@\delim@name#1}}
\def\paireddelim#1{\csuse{delim@close@\delim@name#1}}

\newtoks\delimited@toks
\def\lrify{\@ifnextchar[{\@lrify}{\@@lrify[-]}}
\def\@lrify[#1]{\@iflropt{#1}{\@@lrify[#1]}{\lr[-][]{#1}}}
\def\@@lrify[#1]#2{%
  \ifblank{#2}{}{%
    \ifpaireddelim{#2}{%
      \edef\lrify@lr{\unexpanded{\lr[#1]#2}\paireddelim#2}%
      \collect@delimited@content\lrify@lr#2%
    }{#2}}%
}
% this version fails on {\lrify[contents]}
% \newcommand\lrify[2][-]{%
%   \ifblank{#2}{}{%
%     \@iflropt{#1}{%
%       \ifpaireddelim{#2}{%
%         \edef\lrify@lr{\unexpanded{\lr[#1]#2}\paireddelim#2}%
%         \collect@delimited@content\lrify@lr#2%
%       }{#2}}{%
%       \lr[-][]{#1}#2%
%     }%
% }}

\newcommand\collect@delimited@content[2]{%
  \def\delim@action{#1{\the\delimited@toks}}%
  \begingroup%
  \delimited@toks={}%
  \aftergroup\delim@action%
  \csuse{delim@scantoclose@\delim@name#2}%
}

\def\DeclareLRifiedOperator#1#2{\def#1{\operatorname{#2}\afterscripts\lrify}}
\def\LRifyOperator#1{\cslet{unlrified@\string#1}{#1}\def#1{\csuse{unlrified@\string#1}\afterscripts\lrify}}

\DeclareLRifiedOperator\expect{\mathbb{E}}

  
\makeatother


% LaTeX and amsmath delimiters from Comprehensive Symbol List tables 214-216
\DeclareLRDelimPair()
\DeclareLRDelimPair[]
\DeclareLRDelimPair\{\}
\DeclareLRDelimPair\langle\rangle
\DeclareLRDelimPair\lceil\rceil
\DeclareLRDelimPair\lfloor\rfloor
\DeclareLRDelimPair||
\DeclareLRDelimPair\|\|
\DeclareLRDelimPair\vert\vert
\DeclareLRDelimPair\Vert\Vert
\DeclareLRDelimPair//
\DeclareLRDelimPair\backslash\backslash
\DeclareLRDelimPair\downarrow\downarrow
\DeclareLRDelimPair\Downarrow\Downarrow
\DeclareLRDelimPair\uparrow\uparrow
\DeclareLRDelimPair\Uparrow\Uparrow

\DeclareLRDelimPair\lmoustache\rmoustache
\DeclareLRDelimPair\lgroup\rgroup
\DeclareLRDelimPair\arrowvert\arrowvert
\DeclareLRDelimPair\Arrowvert\Arrowvert
\DeclareLRDelimPair\bracevert\bracevert

\DeclareLRDelimPair\lvert\rvert
\DeclareLRDelimPair\lVert\rVert

% \makeatletter
% \newcommand\lr[4][]{%
%   \ifthenelse{\equal{#1{}}{{}}}%
%              {\def\@lrcontent{#4}%
%                \mathopen{\left#2\vphantom\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
%              {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
% }
% \makeatother

% % old version -- use \lrset( \lrset) in place of \left( right).  Cannot be nested!!
% \newboolean{inlr}
% \newboolean{midlr}
% \setboolean{inlr}{false}
% \newcommand\newlr{\setboolean{inlr}{false}}
% 
% \newcommand\lrset[1]{%
%   \ifthenelse{\boolean{inlr}}%
%     {\ifthenelse{\boolean{midlr}}%
%       {\middle#1\setboolean{inlr}{true}}
%       {\right#1}}%
%     {\left#1\setboolean{inlr}{true}}}%
% \newcommand\lrmid{%
%   \ifthenelse{\boolean{inlr}}%
%     {\setboolean{midlr}{true}}
%     {}}%




% Local Variables:
% mode: latex
% eval: (set-fill-column 120)
% eval: (face-remap-add-relative 'default :family "Ubuntu Mono")
% End:


==> math_commands.tex <==
%!TEX root = ./main.tex

\usepackage{bm,amssymb,amsmath}

% Make theorem titles bold
\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother

\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
% \def\vmu{{\mathbf{\mu}}}
\def\vmu{{\boldsymbol{\mu}}}
\def\vtheta{{\boldsymbol{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\boldsymbol{\beta}}}
\def\mPhi{{\boldsymbol{\Phi}}}
\def\mLambda{{\boldsymbol{\Lambda}}}
\def\mSigma{{\boldsymbol{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\widehat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\widehat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\widetilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\widetilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


